Advancing Multi-Secant Quasi-Newton Methods for General Convex Functions

Quasi-Newton (QN) methods provide an efficient alternative to second-order methods for minimizing smooth unconstrained problems. While QN methods generally compose a Hessian estimate based on one secant interpolation per iteration, multisecant methods use multiple secant interpolations and can improve the quality of the Hessian estimate at small additional overhead cost. However, implementing multisecant QN methods has several key challenges involving method stability, the most critical of which is that when the objective function is convex but not quadratic, the Hessian approximate is not, in general, symmetric positive semidefinite (PSD), and the steps are not guaranteed to be descent directions. We therefore investigate a symmetrized and PSD-perturbed Hessian approximation method for multisecant QN. We offer an efficiently computable method for producing the PSD perturbation, show superlinear convergence of the new method, and demonstrate improved numerical experiments over general convex minimization problems. We also investigate the limited memory extension of the method, focusing on BFGS, on both convex and non-convex functions. Our results suggest that in ill-conditioned optimization landscapes, leveraging multiple secants can accelerate convergence and yield higher-quality solutions compared to traditional single-secant methods.

==> Chapters/App_linear_alg_facts.tex <==


\subsection{Linear algebra facts}
In this section, we review a few key facts from matrix linear algebra, that we use in the design of our algorithm.
%The Schur complement \cite{schurcomplement} is a fundamental concept in the study of block matrices, connecting the properties of the entire matrix to its submatrices. It is particularly useful in analyzing matrix invertibility, definiteness, and determinant computations.
 
Let \( A \) be a block matrix of the form:
\[
A =
\begin{bmatrix}
A_{11} & A_{12} \\
A_{21} & A_{22}
\end{bmatrix},
\]
where \( A_{11} \), \( A_{12} \), \( A_{21} \), and \( A_{22} \) are submatrices. Assume that \( A_{22} \) is invertible. The \textit{Schur complement} of \( A_{22} \) in \( A \) is defined as:
\[
S = A_{11} - A_{12}A_{22}^{-1}A_{21}.
\]
Similarly, if \( A_{11} \) is invertible, the Schur complement of \( A_{11} \) in \( A \) is:
\[
T = A_{22} - A_{21}A_{11}^{-1}A_{12}.
\]

\begin{theorem}[Invertibility]
The block matrix \( A \) is invertible if and only if \( A_{22} \) and its Schur complement \( S \) are invertible. In this case, the inverse of \( A \) can be expressed as:
\[
A^{-1} =
\begin{bmatrix}
S^{-1} & -S^{-1}A_{12}A_{22}^{-1} \\
-A_{22}^{-1}A_{21}S^{-1} & A_{22}^{-1} + A_{22}^{-1}A_{21}S^{-1}A_{12}A_{22}^{-1}
\end{bmatrix}.
\]
\end{theorem}

\begin{theorem}[Definiteness, \citep{zhang2006schur}]
Let \( A_{22} \) be positive definite. Then, \( A \) is positive definite if and only if the Schur complement \( S \) is positive definite.
\end{theorem}


%\begin{proof}
%    Assume \( A \succ 0 \). For \( A \) to be positive definite, it must be symmetric, which ensures that \( A_{11} \), \( A_{22} \), and \( S \) are symmetric. Additionally, determinants of top-left submatrices of \( A \) must be positive. In particular, this implies \( A_{22} \succ 0 \) as a leading principal minor and \( S \succ 0 \) as it governs the definiteness of the remainder of the matrix.

%Conversely, assume \( A_{22} \succ 0 \) and \( S \succ 0 \). To demonstrate that \( A \succ 0 \), consider the quadratic form of \( A \):
%\[
%z^\top A z = 
%\begin{bmatrix}
%x \\
%y
%\end{bmatrix}^\top
%\begin{bmatrix}
%A_{11} & A_{12} \\
%A_{21} & A_{22}
%\end{bmatrix}
%\begin{bmatrix}
%x \\
%y
%\end{bmatrix},
%\]
%where \( x \) and \( y \) are vectors conforming to the %partition of \( A \). Expanding this expression:
%\[
%z^\top A z = x^\top A_{11} x + 2x^\top A_{12} y + y^\top A_{22} y.
%\]
%Completing the square with respect to \( x \), the quadratic form becomes:
%\[
%z^\top A z = (x - A_{12}A_{22}^{-1}y)^\top S (x - A_{12}A_{22}^{-1}y) + y^\top A_{22} y.
%\]
%Since \( S \succ 0 \) and \( A_{22} \succ 0 \), both terms in the above expression are strictly positive for all \( z \neq 0 \). Therefore, \( z^\top A z > 0 \), proving that \( A \succ 0 \).
%\end{proof}

%\begin{theorem}[Determinants]
%The determinant of \( A \) can be expressed as:
%\[
%\det(A) = \det(A_{22}) \cdot \det(S).
%\]
%\end{theorem}
\iffalse

The Schur Complement Theorem provides a powerful result for analyzing the positive definiteness of block matrices. Consider the block matrix
\[
A =
\begin{bmatrix}
A_{11} & A_{12} \\
A_{21} & A_{22}
\end{bmatrix},
\]
where \( A_{11} \), \( A_{12} \), \( A_{21} \), and \( A_{22} \) are submatrices. Assume that \( A_{22} \succ 0 \), i.e., \( A_{22} \) is positive definite. The matrix \( A \) is positive definite (\( A \succ 0 \)) if and only if the Schur complement of \( A_{22} \) in \( A \),
\[
S = A_{11} - A_{12}A_{22}^{-1}A_{21},
\]
is positive definite (\( S \succ 0 \)). The positive definiteness of \( A \) depends on the interplay between \( A_{22} \) and the Schur complement \( S \). The condition \( A_{22} \succ 0 \) ensures that the bottom-right block of \( A \) contributes positively, while \( S \succ 0 \) guarantees the top-left block \( A_{11} \), adjusted for the interaction with \( A_{12} \) and \( A_{21} \), is also positive definite. Together, these conditions ensure the overall positive definiteness of \( A \).
\fi

\iffalse
\begin{lemma}[Conditions for positive definiteness of the Schur Complement ]
\label{lemma:schur_relationship}
    Given the symmetric matrix $ X = 
\begin{bmatrix}
    A&B \\  B^T&C
\end{bmatrix}$, we have the following relationship for the block matrices : 
\begin{itemize}
    \item If $A$ is invertible, then $\quad X\succ 0 \;\iff\; A\succ 0 \quad\text{and}\quad C-B^TA^{-1}B \succ 0$ 
    \item If $C$ is invertible, then $\quad X\succ 0 \;\iff\; C\succ 0\quad\text{and}\quad A-BC^{-1}B^T \succ 0$
    \item If \;$A\succ 0$, then $\quad X\succ 0 \;\iff \; C-B^TA^{-1}B \succeq 0$
    \item If $\;C\succ 0$, then $\quad X\succ 0 \;\iff \; C-B^TA^{-1}B \succeq 0$
\end{itemize}


\end{lemma}
\fi


==> Chapters/App_lowrank_update.tex <==
\section{Estimating $\mu$}\label{sec:app:computemu}
In this section, we give the proof for Theorem \ref{th:lowrankupdate}, which is used to justify our estimate of $\mu$.



 


\begin{theorem}
\label{th:lowrankupdate-restate}
Consider $W$ a nonsymmetric matrix, $c>0$ and 
\begin{equation}
 \Delta =  \frac{1}{2} 
    \begin{bmatrix} D_{1} & D_{2} \end{bmatrix}
    \begin{bmatrix} 0 & W^{-1} \\ W^{-T} & 0 \end{bmatrix}
    \begin{bmatrix}D_{1}^T \\ D_{2}^T \end{bmatrix} \in\mathbb{R}^{n\times n}.
    \label{eq:deltadef:app}
\end{equation}
Then $\Delta + \mu I$ is PSD if and only if 
\begin{equation}
H_2 = \begin{bmatrix}
  cI &  F\\
 F^T& cI
\end{bmatrix}- 
(2\mu)^{-1} G + (2\mu)^{-1}     
G
(2\mu C^{-1}+ G )^{-1}
G 
\label{eq:nonsym_testmat}
\end{equation}
is PSD, for  
    \[C = \begin{bmatrix} (cI - c^{-1}FF^T)^{-1} & W^{-1}-c^{-1}F  (cI - c^{-1}F^TF)^{-1}  \\ W^{-T}-c^{-1} (cI - c^{-1}F^TF)^{-1}  F^T & (cI - c^{-1}F^TF)^{-1} \end{bmatrix},
    \]
$G = \begin{bmatrix} D_1^T \\  D_2^T\end{bmatrix} \begin{bmatrix} D_1 &  D_2\end{bmatrix}$,  $F =  VSU^T$ where $W = U\Sigma V^T$ is the SVD of $W^{-1}$, and $S_{i,i} = \frac{-1+\sqrt{1+4c^2\Sigma_{ii}^{-2}}}{2\Sigma_{i,i}^{-1}}$.
 
\end{theorem}
\begin{proof}
Compare against 
\[
H = \begin{bmatrix}2 \mu I + A & D_1 & D_2 \\ D_1^T & cI & F\\D_2^T & F^T & cI\end{bmatrix}
\]

Then one Schur complement of $H$ is 
\[
H_1 := 2\mu I + A - \begin{bmatrix} D_1 &  D_2\end{bmatrix}\begin{bmatrix} cI & F \\ F^T & cI \end{bmatrix}^{-1} \begin{bmatrix} D_1^T \\  D_2^T\end{bmatrix}
\]
and another is $H_2$ (to be shown later).
So, $H$ is PSD if \begin{itemize}
    \item $A+2\mu I$ is PSD and $H_2$ is PSD
    \item $\begin{bmatrix} cI & F \\ F^T & cI \end{bmatrix}$ is PSD and $H_1$ is PSD
\end{itemize}

Here, $H_1 = 2\Gamma$ if 
\begin{eqnarray*}
A &=&  \begin{bmatrix} D_1 &  D_2\end{bmatrix}\begin{bmatrix} cI & F \\ F^T & cI \end{bmatrix}^{-1} \begin{bmatrix} D_1^T \\  D_2^T\end{bmatrix} +  \begin{bmatrix} D_1 &  D_2 \end{bmatrix}
    \begin{bmatrix} 0 & W^{-1} \\ W^{-T} & 0 \end{bmatrix}
    \begin{bmatrix}D_1^T \\ D_2^T \end{bmatrix} \\
    &=&  \begin{bmatrix} D_1 &  D_2\end{bmatrix}
    \underbrace{\begin{bmatrix} (cI - c^{-1}FF^T)^{-1} & W^{-1}-c^{-1}F  (cI - c^{-1}F^TF)^{-1}  \\ W^{-T}-c^{-1} (cI - c^{-1}F^TF)^{-1}  F^T & (cI - c^{-1}F^TF)^{-1} \end{bmatrix}}_{=:C}
    \begin{bmatrix} D_1^T \\  D_2^T\end{bmatrix}.  
\end{eqnarray*}

We construct $F$ to have the same left and right singular vectors as $W$, so $W = U\Sigma V^T$ and $F = USV^T$. Then   the eigenvalues of $A$ are the same as that of 
 \begin{eqnarray*}
 &&\begin{bmatrix} U^T & 0 \\ 0 & V^T\end{bmatrix} \begin{bmatrix} (cI - c^{-1}FF^T)^{-1} & W^{-1}-c^{-1}F  (cI - c^{-1}F^TF)^{-1}  \\ W^{-T}-c^{-1} (cI - c^{-1}F^TF)^{-1}  F^T & (cI - c^{-1}F^TF)^{-1} \end{bmatrix}\begin{bmatrix} U & 0 \\ 0 & V\end{bmatrix}\\&=&
\begin{bmatrix} (cI - c^{-1}S^2)^{-1} & \Sigma^{-1}-c^{-1}S  (cI - c^{-1}S^2)^{-1}  \\ \Sigma^{-1}-c^{-1} (cI - c^{-1}S^2)^{-1}  S & (cI - c^{-1}S^2)^{-1} \end{bmatrix}\\
 \end{eqnarray*}
 which can be rearranged into a block diagonal matrix whose 2x2 blocks are 
 \[
 B_i = \begin{bmatrix} (c - c^{-1}S_{ii}^2)^{-1} & \Sigma_{ii}^{-1}-c^{-1}S_{ii}  (c - c^{-1}S_{ii}^2)^{-1}  \\ \Sigma_{ii}^{-1}-c^{-1} (c - c^{-1}S_{ii}^2)^{-1}  S_{ii} & (c - c^{-1}S_{ii}^2)^{-1} \end{bmatrix}
 \]
These blocks are PSD if $S_{ii}<c$ and
\begin{eqnarray*}
0&<&
(c - c^{-1}S_{ii}^2)^{-1}   - \frac{(\Sigma_{ii}^{-1}-c^{-1}S_{ii}  (c - c^{-1}S_{ii}^2)^{-1}  )^2}{(c - c^{-1}S_{ii}^2)^{-1}}  \\
\iff && |\Sigma_{ii}^{-1}-\frac{S_{ii}}{c^2 - S_{ii}^2} |<(c - c^{-1}S_{ii}^2)\\
\iff && \Sigma_{ii}^{-1}-\frac{S_{ii}}{c^2 - S_{ii}^2} <(c - c^{-1}S_{ii}^2) \text{ or }
 -\Sigma_{ii}^{-1}+\frac{S_{ii}}{c^2 - S_{ii}^2} <(c - c^{-1}S_{ii}^2)\\
\iff &&c \Sigma_{ii}^{-1}(c^2 - S_{ii}^2)-cS_{ii} < (c^2 - S_{ii}^2)^2 \text{ or }
 cS_{ii}-c\Sigma_{ii}^{-1}(c^2 - S_{ii}^2)  < (c^2 - S_{ii}^2)^2\\
\iff &&S_{ii} > \Sigma_{ii}^{-1}(c^2 - S_{ii}^2)   - c^{-1}(c^2 - S_{ii}^2)^2 \text{ or }
 S_{ii}  < c^{-1}(c^2 - S_{ii}^2)^2 + \Sigma_{ii}^{-1}(c^2 - S_{ii}^2)\\
\iff &&S_{ii} > (c^2 - S_{ii}^2) (\Sigma_{ii}^{-1}  - c^{-1}(c^2 - S_{ii}^2)) \text{ or }
 S_{ii}  <   (\Sigma_{ii}^{-1} + c^{-1}(c^2-S_{ii}^2))(c^2 - S_{ii}^2)
\end{eqnarray*}
which is satisfied if 
\[
S_{ii} =  (c^2 - S_{ii}^2) \Sigma_{ii}^{-1}   \quad \iff \quad S_{i,i} = \frac{-1+\sqrt{1+4c^2\Sigma_{ii}^{-2}}}{2\Sigma_{i,i}^{-1}}\leq \frac{\sqrt{4c^2\Sigma_{ii}^{-2}}}{2\Sigma_{i,i}^{-1}} = c.
\]
 Note that  $\begin{bmatrix} cI & F \\ F^T & cI \end{bmatrix}$ is PSD whenever $ c > 0$ and the Schur complement $\frac{1}{c}(c^2I-F^TF)  \succeq 0 $. Since $\|F^TF\|_2 = c^2\|S\|^2_2 \leq \max_i\, c^4$ then this property holds whenever $  c<1$.

Finally, we show that the expansion of $H_2$ is as written in the theorem statement; specifically, 
\begin{eqnarray*}
H_2&=& \begin{bmatrix}
  cI &  F\\
 F^T& cI
\end{bmatrix}-\begin{bmatrix} D_1^T \\ D_2^T\end{bmatrix} (A+2\mu I)^{-1}\begin{bmatrix} D_1 & D_2\end{bmatrix} \\
&=& \begin{bmatrix}
  cI &  F\\
 F^T& cI
\end{bmatrix}- 
\left(
(2\mu)^{-1} G - (2\mu)^{-1}     
G
(2\mu C^{-1}+ G )^{-1}
G \right)\\
\end{eqnarray*}
for $G = \begin{bmatrix} D_1^T \\  D_2^T\end{bmatrix} \begin{bmatrix} D_1 &  D_2\end{bmatrix}$.



\end{proof}



\iffalse
\begin{lemma}
\label{lem:psd_nonsymm_update-helper1}
Define $c = c_1=c_2$ and
\[
 P = (cI - c^{-1}FF^T)^{-1} , \qquad
 Q = (cI - c^{-1} F^TF)^{-1} 
\]
%\[
%Q =  \frac{1}{c}I + \frac{1}{c^2}F^T(cI-\frac{1}{c}FF^T)^{-1}F
%\]
Pick $F = c_3USV^T$ where $W^{-1} = U\Sigma V^T$ is the full SVD of $W^{-1}$, and $S$ is a diagonal matrix satisfying 
\begin{equation}
\Sigma =  (S^2-c^2I)^{-1} S. 
\label{eq:singvalF}
\end{equation}
Pick $c_3 = \frac{c\epsilon }{c+\|W\|_2}$ for some $\epsilon \in (0,1)$.
Then the inverse
    \[
\begin{bmatrix}
    P &  -F(c^2I- F^TF)^{-1}  \\  -(c^2I- F^TF)^{-1}F^T  & Q
\end{bmatrix}
=\begin{bmatrix}
  cI &  F\\
 { F}^T& c I
\end{bmatrix}^{-1}
\]
Then the following three statements are equivalently true.
\begin{enumerate}
    \item 
$\|F\|_2\leq c$\\

\item $\begin{bmatrix}
  cI &  F\\
 F^T& cI
\end{bmatrix}$ is  PSD\\ 

\item $P$ and $Q$ exists and are also PSD
\end{enumerate}

\end{lemma}




\begin{proof}

Recall the inverse of a 2x2 block matrix can be written as 
\[
\begin{bmatrix}
 cI &  F\\
 { F}^T&cI
\end{bmatrix}^{-1}
=\begin{bmatrix}
  (cI - c^{-1}FF^T)^{-1} &  -F(c^2I- F^TF)^{-1}  \\  -(c^2I- F^TF)^{-1}F^T  & (cI - c^{-1} F^TF)^{-1}
\end{bmatrix}. 
\]

Thus gives the correct construction of $P$ and $Q$.
Then, in the off diagonal terms, 
\begin{eqnarray*}
 -F(c^2I- F^TF)^{-1}
 &=&
  -c_3US V^T(c^2VV^T- c_3^2VS^2 V^T)^{-1} \\
  % &=& -U(c^2U- c_3^2US^2 )^{-1}US V^T \\
  &=&  c_3US(c_3^2S^2-c^2I )^{-1}V^T
\end{eqnarray*}
and
\begin{eqnarray*}
 -(c^2I- F^TF)^{-1}F^T
 &=&
  -(c^2I- c_3^2VS^2 V^T)^{-1}c_3VS U^T \\
  % &=& -U(c^2U- c_3^2US^2 )^{-1}US V^T \\
  &=&  V(c_3^2S^2-c^2I )^{-1} c_3S U^T
  %&=& W^{-1} + c_1c_2(1-\frac{1}{c_3^2})USV^T
\end{eqnarray*}

 Note that 
\[
\Sigma =  (S^2-c^2I)^{-1} S
\iff
(S^2-c^2I)\Sigma  = S
\iff
S_{ii}^2\Sigma_i-S_{ii}-\Sigma_i c^2 = 0 \text{ for } \forall i
\]
and
from the quadratic formula, we have the singular values of $F$ as 
\[
S_{ii} = \frac{1+\sqrt{1+4\Sigma_i^2c^2}}{2\Sigma_i} \leq \frac{1+\sqrt{1}+\sqrt{4\Sigma_i^2c^2}}{2\Sigma_i} = \frac{1}{\Sigma_i}+c 
\]
or, $\frac{1}{c_3}\|F\|_2  \leq c +\|W\|_2$ because $\|F\|_2 = c_3\|S\|_2 $ and $\|F\|_2  \leq (c +\|W\|_2)c_3 = c\epsilon \leq c$. Thus 1. is true under our assignment of $c_3$.\\


Next, we can simply prove the second and third properties by the Schur-complement
\begin{eqnarray*}
\begin{bmatrix}
  cI &  F\\
 F^T& cI
\end{bmatrix}
\succeq 0
&\iff& cI\succeq0 \text{  and  }
cI-\frac{1}{c}FF^T = 
\frac{1}{c}(c^2I-FF^T)  \succeq 0 \\
&\iff& cI\succeq0 \text{  and  }
cI-\frac{1}{c}F^TF = 
\frac{1}{c}(c^2I-F^TF)  \succeq 0 
\end{eqnarray*}
if and only if 
\[
c^2-\|F\|_2^2 \geq 0 \iff \|F\|_2 \leq c.
\] 
\end{proof}





\begin{lemma}
    For any choice of positive number $c$, The matrix 
    \[
    A := \Delta  -2\mu I+ \begin{bmatrix} D_1 & D_2 \end{bmatrix} \begin{bmatrix} c I & F \\ F^{T} & cI \end{bmatrix}^{-1} \begin{bmatrix} D_1^T \\ D_2^T\end{bmatrix}
    \]
    is positive semidefinite.
\end{lemma}

    
\begin{proof}
    Based on our construction, $A$ can be written as

\begin{eqnarray*}
A  &=&   \begin{bmatrix} D_1 & D_2 \end{bmatrix}
\begin{bmatrix}
    (cI - c^{-1}FF^T)^{-1} &  -F(c^2I- F^TF)^{-1} -W^{-1} \\  -(c^2I- F^TF)^{-1}F^T-W^{-T}  & (cI - c^{-1} F^TF)^{-1}
\end{bmatrix}
\begin{bmatrix}  D_1^T \\  D_2^T  \end{bmatrix}\\
   &=& \begin{bmatrix} D_1 U & D_2 V \end{bmatrix}
\underbrace{\begin{bmatrix}
    (cI - c^{-1}c_3^2 S^2 )^{-1} &  c_3S( c_3^2 S^2 -c^2I)^{-1}  -\Sigma  \\  c_3 ( c_3^2 S^2-c^2I)^{-1}S-\Sigma   & (cI - c^{-1} c_3^2S^2)^{-1}
\end{bmatrix}}_{=:B }
\begin{bmatrix}U^T D_1^T \\ V^T D_2^T \end{bmatrix}
\end{eqnarray*}
where $W^{-1} = U\Sigma V^T$ and $F = c_3USV^T$. We are left to show if $B$ is PSD. Note that we may partition $B$ into 4 blocks of diagonal matrices, which means there exists a permutation $PBP^T$ which is block diagonal, with 2x2 symmetric blocks
\[
B_{ii} = \begin{bmatrix} \frac{1}{c-\tfrac{1}{c}c_3^2S_{ii}^2} & \frac{c_3 S_{ii}}{c_3^2 S_{ii}^2 - c^2} - \Sigma_{ii} \\ \frac{c_3 S_{ii}}{c_3^2 S_{ii}^2 - c^2} - \Sigma_{ii} & \frac{1}{c-\tfrac{1}{c} c_3^2 S_{ii}^2}.
\end{bmatrix}
\]
The (1,1) and (2,2) blocks can be shown to be positive since
\begin{equation}
c_3 S_{ii} \leq \frac{c}{c+\|W\|_2} (\|W\|_2 + c) = c.
\label{eq:lem-helper-2}
\end{equation}
Therefore, $B_{ii}$ is PSD iff the (2,1) element has magnitude smaller than both diagonal elements; that is, 
\[
B_{ii} \succeq 0 \iff  \frac{1}{c-\tfrac{1}{c}c_3^2S_{ii}^2} \geq \frac{c_3 S_{ii}}{c_3^2 S_{ii}^2 - c^2} - \Sigma_{ii}.
\]
Since \eqref{eq:lem-helper-2}, this is equivalent to
\[
  c\geq -c_3 S_{ii} -\underbrace{(c^2-c_3^2 S_{ii}^2  ) }_{\geq 0}\Sigma_{ii}
\]
which is true since the right hand side is negative.


\end{proof}


We now provide the main theorem that describes how to compute $\mu$ using only low rank updates by Schur Complement. Note that $A$, $c$, and $F$ are explicitly chosen such that $H_1 = \Delta$ in the following Theorem \ref{th:lowrankupdate}. 

\begin{theorem}
\label{th:lowrankupdate}
Consider $W$ a nonsymmetric matrix, $c>0$ and 
\begin{equation}
 \Gamma =
\mu I
+ \frac{1}{2} 
    \begin{bmatrix} D_1 &  D_2 \end{bmatrix}
    \begin{bmatrix} 0 & W^{-1} \\ W^{-T} & 0 \end{bmatrix}
    \begin{bmatrix}D_1^T \\ D_2^T \end{bmatrix}  .
    \label{eq:deltadef:app}
\end{equation}

Then $\Gamma$ is PSD if and only if 
\begin{equation}
H_2 = \begin{bmatrix}
  cI &  F\\
 F^T& cI
\end{bmatrix}
-
\begin{bmatrix} D_1^T \\ D_2^T\end{bmatrix} (A+2\mu I)^{-1}\begin{bmatrix} D_1 & D_2\end{bmatrix} .
\label{eq:nonsym_testmat}
\end{equation}
is PSD, for 
\[
A = %D_1(cI - c^{-1}FF^T)^{-1}D_1^T + D_2 (cI - c^{-1} F^TF)^{-1}D_2^T
    \begin{bmatrix} D_1 & D_2 \end{bmatrix}
\begin{bmatrix}
    P &  -(c^2I- F^TF)^{-1}F^{T} +W^{-1} \\  -F(c^2I- F^TF)^{-1}+W^{-T}  & Q
\end{bmatrix}
\begin{bmatrix} D_1^T \\ D_2^T \end{bmatrix}\\
\]
%\red{
%\[
%\begin{bmatrix}
%(cI-\frac{1}{c}FF^T)^{-1}=P  & -(c^2 I-FF^T)^{-1}F)-W^{-1} \\
 %-F^T(c^2I- F^TF)^{-1}-W^{-T} & \frac{1}{c}I + \frac{1}{c}F^T(c^2I-FF^T)^{-1}F=Q
%\end{bmatrix}
%\]
%}

and $F = \frac{c\epsilon }{c+\|W\|_2} VSU^T$ where $W^{-1} = U\Sigma V^T$ is the SVD of $W^{-1}$, and $S$ is a diagonal matrix satisfying 
\eqref{eq:singvalF}.

\end{theorem}



\begin{proof}
Consider the matrix
\[ 
H = 
\begin{bmatrix}
2\mu I+A & D_1 & D_2\\
D_1^T & cI & F\\
D_2^T & F^T & cI
\end{bmatrix}.
\]
where $c$ is a nonnegative scalar, $F$ is a $2p\times 2p$ matrix (yet undefined), and $A$ is some (unspecified) symmetric matrix.
Then the two Schur complements of $H$ are 
$H_1$ and $H_2$:
\begin{eqnarray*}
H_1&:=&2\mu  I + A - \begin{bmatrix} D_1 & D_2\end{bmatrix} 
\begin{bmatrix}
  cI &  F\\
 { F}^T& c I
\end{bmatrix}^{-1}
\begin{bmatrix} D_1^T \\ D_2^T\end{bmatrix}\in\mathbb{R}^{n\times n} \\
H_2&=&
\underbrace{\begin{bmatrix}
  cI &  F\\
 F^T& cI
\end{bmatrix}}_{H_3}
-
\begin{bmatrix} D_1^T \\ D_2^T\end{bmatrix} (A+2\mu I)^{-1}\begin{bmatrix} D_1 & D_2\end{bmatrix}\in\mathbb{R}^{4m\times 4m}.
\end{eqnarray*}
Then, 
\begin{center}
    $H_1$ is PSD and $\begin{bmatrix}
  c_1I &  F\\
 F^T& c_2I
\end{bmatrix}$ is PSD and invertible
\end{center}
if and only if 
\begin{center}
    $H_2$ is PSD  and $A+2\mu I$ is PSD and invertible.
\end{center}

From Lemma \ref{lem:psd_nonsymm_update-helper1}, we see that the proposed construction of $A$ and $F$ is indeed valid for setting $\Gamma = H_1$; moreover, for any value of $c > 0$, $A$ and $H_3$ are both PSD. Thus, $\Gamma$ is PSD if and only if $H_2$ is PSD.

\end{proof}


Note that while we have pushed the certification of PSD from our original $n\times n$ matrix $\Delta$ to that of a smaller $2p\times 2p$ matrix in \eqref{eq:nonsym_testmat}, the inversion $(A+2\mu I)^{-1}\in \R^{n\times n}$ still seems daunting. However, note that
\[
A+2\mu I = \begin{bmatrix} D_1 & D_2 \end{bmatrix} B
\begin{bmatrix} D_1^T \\ D_2^T \end{bmatrix}
+ 2\mu I
\]
for
\[
B = 
\begin{bmatrix}
    (cI - c^{-1}FF^T)^{-1} &  -(c^2I- F^TF)^{-1}F^{T} +W^{-1} \\  -F(c^2I- F^TF)^{-1}+W^{-T}  & (cI - c^{-1} F^TF)^{-1}
\end{bmatrix} \in\mathbb{R}^{4m\times 4m}
\]
is a diagonal-plus-low-rank matrix, and its inverse can be efficiently computed using another Woodbury inversion
\[
(A+2\mu I)^{-1} = \frac{1}{ 2\mu} I- \frac{1}{2\mu} \begin{bmatrix} D_1 & D_2 \end{bmatrix}\left(2\mu B^{-1}  + \begin{bmatrix} D_1^T \\ D_2^T \end{bmatrix} \begin{bmatrix} D_1 & D_2 \end{bmatrix} \right)^{-1}\begin{bmatrix} D_1^T \\ D_2^T \end{bmatrix}.
\]






\fi









\iffalse
 \ref{th:lowrankupdate}. 
\begin{theorem}
\label{th:lowrankupdate}
Consider $W$ a nonsymmetric matrix, and 
\begin{equation}
 \Delta =
\mu I
- \frac{1}{2} 
    \begin{bmatrix} D_1 &  D_2 \end{bmatrix}
    \begin{bmatrix} 0 & W^{-1} \\ W^{-T} & 0 \end{bmatrix}
    \begin{bmatrix}D_1^T \\ D_2^T \end{bmatrix}.
    \label{eq:deltadef}
    \end{equation}
We take the eigenvalue decomposition of the $p\times p$ matrix
$W^{-1} = U\Sigma V^T$, and for any $c 
> 0$, $0\leq \epsilon \leq 1$, construct
\begin{align}
\Sigma =  (S^2-c^2I)^{-1} S, \qquad
 F = \frac{c\epsilon }{c+\|W\|_2} VSU^T,\\
 P = (cI - c^{-1}FF^T)^{-1},\qquad
 Q = (cI - c^{-1} F^TF)^{-1},\\
  A =
    \begin{bmatrix} D_1 & D_2 \end{bmatrix}
\begin{bmatrix}
    P &  -cQF^{T} -W^{-1} \\  -cFQ-W^{-T}  & Q
\end{bmatrix}
\begin{bmatrix} D_1^T \\ D_2^T \end{bmatrix}.
 \label{eq:mupsd-vardef}
\end{align}
Then $\Delta$ is PSD if and only if 
\begin{equation*}
H_2 = \begin{bmatrix}
  cI &  F\\
 F^T& cI
\end{bmatrix}
-
\begin{bmatrix} D_1^T \\ D_2^T\end{bmatrix} (A+2\mu I)^{-1}\begin{bmatrix} D_1 & D_2\end{bmatrix}
\label{eq:nonsym_testmat}
\end{equation*}
is PSD. 
\end{theorem}


\begin{proof}[Proof of Thm. \ref{th:lowrankupdate}]
    First, we verify that by this construction, 
    \[
 A =
    \begin{bmatrix} D_1 & D_2 \end{bmatrix}
\begin{bmatrix}
    P &  -cQF^{T} -W^{-1} \\  -cFQ-W^{-T}  & Q
\end{bmatrix}
\begin{bmatrix} D_1^T \\ D_2^T \end{bmatrix}.
\]
is PSD. 
    Based on our construction, $A$ can be written as

\begin{align*}
A  &=   \begin{bmatrix} D_1 & D_2 \end{bmatrix}
\begin{bmatrix}
    P &  -c
    FQ-W^{-1} \\  -cQF^T-W^{-T}  & Q
\end{bmatrix}
\begin{bmatrix}  D_1^T \\  D_2^T  \end{bmatrix}\\
   &= \begin{bmatrix} D_1 U & D_2 V \end{bmatrix}
\underbrace{\begin{bmatrix}
    R &  -c\delta SR  -\Sigma  \\ -c \delta R S-\Sigma   & R
\end{bmatrix}}_{\Huge{:= \; E \;\in \;\mathbb{R}^{2p\times 2p}} }
\begin{bmatrix}U^T D_1^T \\ V^T D_2^T \end{bmatrix}
\end{align*}
where 
\[
R = (cI - c^{-1}\delta^2 S^2 )^{-1}, \qquad \delta =  \frac{c\epsilon }{c+\|W\|_2}.
\]
Also, from \eqref{eq:mupsd-vardef}, the first equation is a quadratic equation involving $S_{ii}$ satisfying
\[
S_{ii} = \frac{1+\sqrt{1+4\Sigma_i^2c^2}}{2\Sigma_i} \leq  \frac{1}{\Sigma_i}+c.
\]
Note that since $\Sigma_i$ are the singular values of $W^{-1}$,
 $\frac{1}{\Sigma_i} \leq  \|W\|_2$, which implies $S_{ii} \leq \|W\|_2+c$.
 
We are left to show if $E$ is PSD. Note that we may partition $E$ into 4 blocks of diagonal matrices, which means there exists a permutation $PEP^T$ which is block diagonal, with 2-by-2 symmetric sub-blocks
\[
E_{ii} = \begin{bmatrix} (c-\tfrac{1}{c}\delta^2S_{ii}^2)^{-1} & \frac{\delta S_{ii}}{\delta^2 S_{ii}^2 - c^2} - \Sigma_{ii} \\ \frac{\delta S_{ii}}{\delta^2 S_{ii}^2 - c^2} - \Sigma_{ii} & (c-\tfrac{1}{c} \delta^2 S_{ii}^2)^{-1}
\end{bmatrix}\in\mathbb{R}^{2\times 2}.
\]
The (1,1) and (2,2) blocks can be shown to be positive since
\begin{equation}
\delta S_{ii} \leq \frac{c}{c+\|W\|_2} (\|W\|_2 + c) = c.
\label{eq:lem-helper-2}
\end{equation}
Therefore, $E_{ii}$ is PSD if and only if the (2,1) element has magnitude smaller than both diagonal elements; that is, 
\[
E_{ii} \succeq 0 \iff  \frac{1}{c-\tfrac{1}{c}\delta^2S_{ii}^2} \geq \frac{\delta S_{ii}}{\delta^2 S_{ii}^2 - c^2} - \Sigma_{ii}.
\]
Since \eqref{eq:lem-helper-2}, this is equivalent to
\[
  c\geq -c_3 S_{ii} -\underbrace{(c^2-c_3^2 S_{ii}^2  ) }_{\geq 0}\Sigma_{ii}
\]
which is true since the right hand side is negative.

Next, we consider the matrix $H$ 
\[ 
H = 
\begin{bmatrix}
A+2\mu I & D_1 & D_2\\
D_1^T & cI & F\\
D_2^T & F^T & cI
\end{bmatrix}
\]
where $c$ is a non-negative scalar, $F$ is a $p\times p$ matrix (yet undefined), and $A$ is some (unspecified) symmetric matrix.
Then the two Schur complements of $H$ are 
$H_1$ and $H_2$:
\begin{align*}
H_1& := A+2\mu I - \begin{bmatrix} D_1 & D_2\end{bmatrix} 
\begin{bmatrix}
  cI &  F\\
 { F}^T& c I
\end{bmatrix}^{-1}
\begin{bmatrix} D_1^T \\ D_2^T\end{bmatrix} \in\mathbb{R}^{n\times n}\\
H_2& :=
\begin{bmatrix}
  cI &  F\\
 F^T& cI
\end{bmatrix}
-
\begin{bmatrix} D_1^T \\ D_2^T\end{bmatrix} (A+2\mu I)^{-1}\begin{bmatrix} D_1 & D_2\end{bmatrix} \in\mathbb{R}^{2p\times 2p}
\end{align*}
Then, 
\begin{center}
    $H_1$ is PSD and 
    $\begin{bmatrix}
  cI &  F\\
 F^T& cI
\end{bmatrix}$ 
is PSD and invertible
\end{center}
if and only if 
\begin{center}
    $H_2$ is PSD  and $A+2\mu I$ is PSD and invertible.
\end{center}

Since we already showed that $A$ is PSD, we see that testing $H_2$ for PSD is sufficient to guarantee $H_1$ is PSD.
%the proposed construction of $A$ and $F$ is indeed valid for setting $\Delta = H_1$; moreover, for any value of $c > 0$, $A$ and $H_3$ are both PSD. Thus, $\Delta$ is PSD if and only if $H_2$ is PSD.


\end{proof}

\fi

==> Chapters/App_woodburyinversion.tex <==

\subsection{Woodbury Inversion of Multisecant BFGS}

The four update rules \eqref{eq:MS_Broyden}, \eqref{eq:MS_DFP}, \eqref{eq:MS_PSB},\eqref{eq:MS_BFGS}
 can be succinctly written as 
 \[
 B_{k+1} = B_k + C_kA_kC_k^T
 \]
 where $C_k$ and $A_k$ depend on $B_k$, $S_k$, and $Y_k$. Specifically, the update is \textit{low-rank}; $A_k$ is $p\times p$ for Broyden's method, and $2p\times 2p$ for the others. 
 To avoid computing inverses, low-rank updates of $B_k$ are updated using the Sherman-Morrison-Woodbury inversion lemma \citep{woodbury1950inverting,hager1989updating,lu2002inverses}
 %and the properties of the inverses of $2 \times 2$ block matrices
%\cite{lu2002inverses} 
%where $U$, $C$, and $V$ are the appropriate matrices as in the definitions.
This leads to the following updates for Broyden's method
\[
B_{k+1}^{-1} =  B_k^{-1}-(B_k^{-1}Y_k-S_k)(S_k^T B_k^{-1} Y_k)^{-1}S_k^TB_k^{-1}
\] 
and BFGS
\begin{align*}
B_{k+1}^{-1}  & = B_k^{-1}-(B_k^{-1}Y_k, S_k)
\begin{pmatrix}
Y_k^TS_k+Y_k^TB_k^{-1}Y_k & Y_k^TS_k\\
S_k^TY_k & 0
\end{pmatrix}^{-1}
\begin{pmatrix}
Y_k^TB^{-1}\\ S_k^T
\end{pmatrix}
\end{align*} 
where importantly there is no need to take $n\times n$ matrix inverses.
While we do not need to explicitly symmetrize the BFGS update, it is interesting to note that for this update,
\[
B_{k+1}^{-1}+B_{k+1}^{-1,T}= (B_{k+1}+B_{k+1}^{T})^{-1}.
\]
\paragraph{PSB and DFP inverse updates.}
The inverse updates for PSB and DFP require a few extra adjustments. Specifically, it is not clear how to to completely cancel out the $B_k$ term in the update, which is necessary if we want an inverse-only update. Therefore, assuming $S_k$ has full column rank\footnote{This property is anyway necessary for good convergence of the method, and is ensured using the rejection method in our extensions.}, we first produce 
\[
 S_k^TB_kS_k =  (S_k^{\dagger,T} B_k^{-1} S_k^\dagger)^{-1} 
\]
where $S^\dagger =  (S^TS)^{-1}S^T$ the left-inverse of $S$. 
Then, the symmetrized PSB update
\begin{align}
B_{k+1} &= B_k + (Y_k-B_kS_k)(S_k^TS_k)^{-1}S_k^T + S_k(S_k^TS_k)^{-1}(Y_k-B_kS_k)^T\nonumber\\
&+ S_k (S_k^TS_k)^{-1}S_k^TB_kS(S_k^TS_k)^{-1}S_k^T 
\nonumber\\
&-\frac{1}{2} S_k (S_k^TS_k)^{-1}(Y_k^TS_k +  S_k^TY_k)(S_k^TS_k)^{-1}S_k^T \tag{MS-S-PSB} \label{eq:MS_PSB_symm}
\end{align}
has inverse update
\begin{eqnarray*}
B_{k+1}^{-1} 
=B_k^{-1} - D_{1,k} W_k^{-1} D_{2,k}
\end{eqnarray*}

 


where  for 
\[
D_{1,k} = \begin{bmatrix} B_k^{-1} Y_k - S_k, & B_k^{-1} S_k,& B_k^{-1} S,&B^{-1} S_k\end{bmatrix}, \qquad D_{2,k} = \begin{bmatrix} B_k^{-1} S_k,& B_k^{-1} Y_k - S_k, &  B^{-1} S_k,&B_k^{-1} S\end{bmatrix}, 
\]
and
\[
W_k = \begin{bmatrix}
     S_k^TB_k^{-1}Y_k, & V_k,& V_k, & V_k \\

  X_k,  &   Y_k^T B_k^{-1}S_k&  U_k^T & U_k^T \\

   U_k & V_k&  Z_k +  V_k& V_k\\

   U_k& V_k& V_k&  G_k +  V_k\\
    
\end{bmatrix}
\] 
$U_k = S_k^TB_k^{-1}Y_k - S_k^TS_k$, $V_k = S_k^TB_k^{-1}S_k$,  
$X_k = Y_k^TB_k^{-1}Y_k - S_k^TY_k - Y_k^TS_k + S_k^TB_kS_k$, $Z_k = S_k^TS_k(S_k^TB_kS_k)^{-1} S_k^TS_k$, 
 $G_k = -\frac{1}{2} S_k^TS_k (Y_k^TS_k  + S_k^TY_k)^{-1} S_k^TS_k $.
Similarly, using a symmetrized DFP update
\begin{align}
B_{k+1} &= B_k + (Y_k-B_kS_k)(Y_k^TS)^{-1}Y^T 
+ Y_k(S_k^TY_k)^{-1}(Y_k-BS)^T \nonumber\\&
 + Y_k(S_k^TY_k)^{-1}S_k^TB_kS_k(Y_k^TS_k)^{-1} Y^T
  - \frac{1}{2}Y((S_k^TY_k)^{-1} + (Y_k^TS_k)^{-1})  Y^T\tag{MS-S-DFP} \label{eq:MS_DFP_symm}
\end{align}
then for  $R_k = Y_k^TS_k$, $H_k =  S_k^TB_kS_k$, $Q_k = B_k^{-1}Y_k$, and $T_k = Y_k^TB_k^{-1}Y_k$,
\begin{eqnarray*}
B_{k+1}^{-1} 
  &=& B^{-1} -  \begin{bmatrix} Q_k-S_k,&Q_k,&Q_k  \end{bmatrix} \begin{bmatrix}
       T_k ,&T_k,&T_k\\ 
      T_k - R_k^T - R_k + H_k, & R_k +T_k  - R_k^T,&T_k - R_k^T\\
      T_k - R_k,&T_k,& -Q_k (Q_k-H_k)^{-1}Q_k + T_k
  \end{bmatrix}^{-1}
  \begin{bmatrix} Q_k^T\\Q_k^T-S_k^T\\Q_k^T\end{bmatrix}.
\end{eqnarray*}
Using these Woodbury inversion updates  significantly reduces computational requirements  from \( O(n^3) \) to \( O(pn^2 + p^3) \). 


Each of the four multisecant methods now has an inverse update which can be written in the form
\begin{equation}
    \hat B^{-1}_{k+1} = B^{-1}_k + D_{1,k} W_k^{-1} D_{2,k}^T 
    \label{eq:summarize_MS}
\end{equation}
where $W_k$ is $p\times p$ for Broyden's method, and $2p\times 2p$ for PSB, DFP, and BFGS.
Note that $W$ is not assumed to be symmetric nor PSD in general.





\begin{table}[H]
    \centering
    \hspace*{-1cm}
    \begin{tabular}[t]{l|ccc}\hline
         & $D_1$ & $D_2$& $W$  \\\hline
      Broyden's   & $Z_k $ & $S_k$ & $-S_k^TS_k\in \R^{p\times p}$ \\[1ex] 
      PSB   & $\begin{bmatrix} Z_k & S_k & S_k\end{bmatrix} $  & $\begin{bmatrix} S_k &  Z_k & S_k\end{bmatrix} $ & $\begin{bmatrix} -S_k^TS_k & 0 & 0\\0 & -S_k^TS_k & 0\\ 0 & 0 & S_k^TS_k(Z_k^TS_k)^{-1}S_k^TS_k
      \end{bmatrix} \in \R^{3p\times 3p}$ \\[5ex]
      DFP   & $\begin{bmatrix} Z_k & Y_k & Y_k\end{bmatrix} $  & $\begin{bmatrix} Y_k &  Z_k & Y_k\end{bmatrix} $ & $\begin{bmatrix} -Y_k^TS_k & 0 & 0\\0 & -Y_k^TS_k & 0\\ 0 & 0 & (Y_k^TS_k)(Z_k^TS_k)^{-1}(Y_k^TS_k) \end{bmatrix} \in \R^{3p\times 3p}$ \\[5ex]
      BFGS   & $\begin{bmatrix} Y_k & B_kS_k\end{bmatrix} $ &  $\begin{bmatrix} Y_k & B_kS_k\end{bmatrix} $ &  $\begin{bmatrix} -Y_k^TS_k & 0\\0 & S_k^TB_kS_k\end{bmatrix} \in \R^{2p\times 2p}$\\[5ex]
BFGS  inv*  & $[H_kY_k\quad S_k]$ & $[H_k^TY_k \quad S_k]$ & $
\begin{bmatrix}
Y_k^TH_kY_k+Y_k^TS & Y_k^TS_k\\
S_k^TY_k & 0
\end{bmatrix} \in \R^{2p\times 2p}  $\\\hline
    \end{tabular}
    \caption{All four multisecant (MS) methods can be written in form \eqref{eq:summarize_MS}, with the following choices of $D_1$, $D_2$, and $W$, where $W$ is related to the Schur complement of the update matrix. Here, we write $Z_k = Y_k-B_kS_k$. We also show the update of $H_k = B^{-1}_k$ for BFGS. *= update is consistent only if $B_k$ is symmetric PSD at each iteration. \red{redo for inverse}}
    \label{tab:QNsummary}
\end{table}


